WIRC+Pol: a low-resolution near-infrared spectropolarimeter

WIRC+Pol is a newly commissioned low-resolution (R~100), near-infrared (J and H band) spectropolarimetry mode of the Wide-field InfraRed Camera (WIRC) on the 200-inch Hale Telescope at Palomar Observatory. The instrument utilizes a novel polarimeter design based on a quarter-wave plate and a polarization grating (PG), which provides full linear polarization measurements (Stokes I, Q, and U) in one exposure. The PG also has high transmission across the J and H bands. The instrument is situated at the prime focus of an equatorially mounted telescope. As a result, the system only has one reflection in the light path, providing minimal telescope induced polarization. A data reduction pipeline has been developed for WIRC+Pol to produce linear polarization measurements from observations. WIRC+Pol has been on-sky since February 2017. Results from the first year commissioning data show that the instrument has a high dispersion efficiency as expected from the polarization grating. We demonstrate the polarimetric stability of the instrument with RMS variation at 0.2% level over 30 minutes for a bright standard star (J = 8.7). While the spectral extraction is photon noise limited, polarization calibration between sources remain limited by systematics, likely related to gravity dependent pointing effects. We discuss instrumental systematics we have uncovered in the data, their potential causes, along with calibrations that are necessary to eliminate them. We describe a modulator upgrade that will eliminate the slowly varying systematics and provide polarimetric accuracy better than 0.1%.

==> old/latexdefs.tex <==
\newcommand\phn{\phantom{0}}% 
\newcommand\phd{\phantom{.}}% 
\newcommand\phs{\phantom{$-$}}% 
\newcommand\phm[1]{\phantom{#1}}% 
\let\la=\lesssim            % For Springer A&A compliance... 
\let\ga=\gtrsim 
\newcommand\sq{\mbox{\rlap{$\sqcap$}$\sqcup$}}% 
\newcommand\arcdeg{\mbox{$^\circ$}}% 
\newcommand\arcmin{\mbox{$^\prime$}}% 
\newcommand\arcsec{\mbox{$^{\prime\prime}$}}% 
\newcommand\fd{\mbox{$.\!\!^{\mathrm d}$}}% 
\newcommand\fh{\mbox{$.\!\!^{\mathrm h}$}}% 
\newcommand\fm{\mbox{$.\!\!^{\mathrm m}$}}% 
\newcommand\fs{\mbox{$.\!\!^{\mathrm s}$}}% 
\newcommand\fdg{\mbox{$.\!\!^\circ$}}% 
\newcommand\fp{\mbox{$.\!\!^{\scriptscriptstyle\mathrm p}$}}% 
\newcommand\micron{\mbox{$\mu$m}}% 
\def\farcm{% 
 \mbox{.\kern -0.7ex\raisebox{.9ex}{\scriptsize$\prime$}}% 
}% 
\def\farcs{% 
 \mbox{% 
  \kern  0.13ex.% 
  \kern -0.95ex\arcsec% 
  \kern -0.1ex% 
 }% 
}% 
%\renewcommand\case[2]{\mbox{$\frac{#1}{#2}$}}% 
%\renewcommand\slantfrac{\case}% 
\newcommand\onehalf{\slantfrac{1}{2}}% 
\newcommand\onethird{\slantfrac{1}{3}}% 
\newcommand\twothirds{\slantfrac{2}{3}}% 
\newcommand\onequarter{\slantfrac{1}{4}}% 
\newcommand\threequarters{\slantfrac{3}{4}}% 
\newcommand\ubvr{\mbox{$U\!BV\!R$}}%% UBVR system 
\newcommand\ub{\mbox{$U\!-\!B$}}%   % U-B 
\newcommand\bv{\mbox{$B\!-\!V$}}%   % B-V 
%\renewcommand\vr{\mbox{$V\!-\!R$}}%   % V-R 
\newcommand\ur{\mbox{$U\!-\!R$}}%   % U-R 
\makeatletter
\newcommand\ion[2]{#1$\;$\protect \textsmaller{\rmfamily\@Roman{#2}}}% 
\newcommand\smion[2]{#1$\;$\protect \footnotesize{\rmfamily\@Roman{#2}}\small}% 
\newcommand\scion[2]{#1$\;$\protect \tiny{\rmfamily\@Roman{#2}}\scriptsize}% 
\makeatother
\newcommand\nodata{ ~$\cdots$~ }% 
\newcommand\diameter{\ooalign{\hfil/\hfil\crcr\mathhexbox20D}}% 
\newcommand\degr{\arcdeg}% 
\newcommand\Sun{\sun}% 
\newcommand\Sol{\sun}% 
\newcommand\sun{\odot}% 
\newcommand\Mercury{\astro{\char1}}% Mercury symbol, "1" 
\newcommand\Venus{\astro{\char2}}% Venus symbol, "2" 
\newcommand\Earth{\earth}% 
\newcommand\Terra{\earth}% 
\newcommand\earth{\oplus}% 
\newcommand\Mars{\astro{\char4}}% Mars symbol, "4" 
\newcommand\Jupiter{\astro{\char5}}% Jupiter symbol, "5" 
\newcommand\Saturn{\astro{\char6}}% Saturn symbol, "6" 
\newcommand\Uranus{\astro{\char7}}% Uranus symbol, "7" 
\newcommand\Neptune{\astro{\char8}}% Neptune symbol, "8" 
\newcommand\Pluto{\astro{\char9}}% Pluo symbol, "9" 
\newcommand\Moon{\astro{\char10}}% Moon symbol, "M" 
\newcommand\Luna{\Moon}% 
\newcommand\Aries{\astro{\char11}}% 
\newcommand\VEq{\Aries}% vernal equinox (Aries) 
\newcommand\Taurus{\astro{\char12}}% 
\newcommand\Gemini{\astro{\char13}}% 
\newcommand\Cancer{\astro{\char14}}% 
\newcommand\Leo{\astro{\char15}}% 
\newcommand\Virgo{\astro{\char16}}% 
\newcommand\Libra{\astro{\char17}}% 
\newcommand\AEq{\Libra}% autumnal equinox (Libra) 
\newcommand\Scorpius{\astro{\char18}}% 
\newcommand\Sagittarius{\astro{\char19}}% 
\newcommand\Capricornus{\astro{\char20}}% 
\newcommand\Aquarius{\astro{\char21}}% 
\newcommand\Pisces{\astro{\char22}}% 

\newcommand\caii{Ca~{\sc ii}}
\newcommand\mgi{Mg~{\sc i}}
\newcommand\fehphot{$\rm{[Fe/H]_{phot}}$}
\newcommand\fehspec{$\rm{[Fe/H]_{spec}}$}
\newcommand\lcdm{$\Lambda$CDM}
\newcommand{\teff}{$T_{\rm{eff}}$}
\newcommand{\mathteff}{T_{\rm{eff}}}
\newcommand{\logg}{$\log g$}
\newcommand{\mathlogg}{\log g}
\newcommand{\feh}{[Fe/H]}
\newcommand{\mathfeh}{\rm{[Fe/H]}}
\newcommand{\afe}{[$\alpha$/Fe]}
\newcommand{\xfe}{[X/Fe]}
\newcommand{\mathafe}{\rm{[\alpha/Fe]}}
\newcommand{\mathxfe}{\rm{[X/Fe]}}
\newcommand{\ah}{[$\alpha$/H]}
\newcommand{\mathah}{\rm{[\alpha/H]}}
\newcommand{\vt}{$v_t$}
\newcommand{\mathvt}{v_t}
\newcommand{\cfht}{\textsc{cfht}}
\newcommand{\ha}{H$\alpha$}
\newcommand{\deep}{\textsc{deep2}}
\newcommand{\deimos}{\textsc{deimos}}
\newcommand{\mathaa}{\mathrm{\AA}}
\newcommand{\ngcaf}{NGC~1904 (M79)}
\newcommand{\ngca}{M79}
\newcommand{\ngcb}{NGC 2419}
\newcommand{\ngccf}{NGC~6205 (M13)}
\newcommand{\ngcc}{M13}
\newcommand{\ngcdf}{NGC~6838 (M71)}
\newcommand{\ngcd}{M71}
\newcommand{\ngce}{NGC 7006}
\newcommand{\ngcff}{NGC~7078 (M15)}
\newcommand{\ngcf}{M15}
\newcommand{\ngcg}{NGC 7492}
\newcommand{\bd}{BD+28$^{\circ}$~4211}

\newcommand{\otoprule}{\midrule[\heavyrulewidth]}
\newcommand\aj{AJ}
          % Astronomical Journal
\newcommand\actaa{Acta Astron.}
  % Acta Astronomica
\newcommand\araa{ARA\&A}
          % Annual Review of Astron and Astrophys
\newcommand\apj{ApJ}
          % Astrophysical Journal
\newcommand\apjl{ApJ}
          % Astrophysical Journal, Letters
\newcommand\apjs{ApJS}
          % Astrophysical Journal, Supplement
\newcommand\ao{Appl.~Opt.}
          % Applied Optics
\newcommand\apss{Ap\&SS}
          % Astrophysics and Space Science
\newcommand\aap{A\&A}
          % Astronomy and Astrophysics
\newcommand\aapr{A\&A~Rev.}
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{A\&AS}
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{AZh}
          % Astronomicheskii Zhurnal
\newcommand\baas{BAAS}
          % Bulletin of the AAS
\newcommand\caa{Chinese Astron. Astrophys.}
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{Chinese J. Astron. Astrophys.}
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{Icarus}
  % Icarus
\newcommand\jcap{J. Cosmology Astropart. Phys.}
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{JRASC}
          % Journal of the RAS of Canada
\newcommand\memras{MmRAS}
          % Memoirs of the RAS
\newcommand\mnras{MNRAS}
          % Monthly Notices of the RAS
\newcommand\na{New A}
  % New Astronomy
\newcommand\nar{New A Rev.}
  % New Astronomy Review
\newcommand\pra{Phys.~Rev.~A}
          % Physical Review A: General Physics
\newcommand\prb{Phys.~Rev.~B}
          % Physical Review B: Solid State
\newcommand\prc{Phys.~Rev.~C}
          % Physical Review C
\newcommand\prd{Phys.~Rev.~D}
          % Physical Review D
\newcommand\pre{Phys.~Rev.~E}
          % Physical Review E
\newcommand\prl{Phys.~Rev.~Lett.}
          % Physical Review Letters
\newcommand\pasa{PASA}
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{PASP}
          % Publications of the ASP
\newcommand\pasj{PASJ}
          % Publications of the ASJ
\newcommand\qjras{QJRAS}
          % Quarterly Journal of the RAS
\newcommand\rmxaa{Rev. Mexicana Astron. Astrofis.}
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{S\&T}
          % Sky and Telescope
\newcommand\solphys{Sol.~Phys.}
          % Solar Physics
\newcommand\sovast{Soviet~Ast.}
          % Soviet Astronomy
\newcommand\ssr{Space~Sci.~Rev.}
          % Space Science Reviews
\newcommand\zap{ZAp}
          % Zeitschrift fuer Astrophysik
\newcommand\nat{Nature}
          % Nature
\newcommand\iaucirc{IAU~Circ.}
          % IAU Cirulars
\newcommand\aplett{Astrophys.~Lett.}
          % Astrophysics Letters and Communications
\newcommand\apspr{Astrophys.~Space~Phys.~Res.}
          % Astrophysics Space Physics Research
\newcommand\bain{Bull.~Astron.~Inst.~Netherlands}
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{Fund.~Cosmic~Phys.}
          % Fundamental Cosmic Physics
\newcommand\gca{Geochim.~Cosmochim.~Acta}
          % Geochimica Cosmochimica Acta
\newcommand\grl{Geophys.~Res.~Lett.}
          % Geophysics Research Letters
\newcommand\jcp{J.~Chem.~Phys.}
          % Journal of Chemical Physics
\newcommand\jgr{J.~Geophys.~Res.}
          % Journal of Geophysical Research
\newcommand\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{Mem.~Soc.~Astron.~Italiana}
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{Nucl.~Phys.~A}
          % Nuclear Physics A
\newcommand\physrep{Phys.~Rep.}
          % Physics Reports
\newcommand\physscr{Phys.~Scr}
          % Physica Scripta
\newcommand\planss{Planet.~Space~Sci.}
          % Planetary Space Science
\newcommand\procspie{Proc.~SPIE}
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
